STRETCH: Virtual Shared-Nothing Parallelism for Scalable and Elastic Stream Processing

Stream processing applications extract value from raw data through Directed Acyclic Graphs of data analysis tasks. Shared-nothing (SN) parallelism is the de-facto standard to scale stream processing applications. Given an application, SN parallelism instantiates several copies of each analysis task, making each instance responsible for a dedicated portion of the overall analysis, and relies on dedicated queues to exchange data among connected instances. On the one hand, SN parallelism can scale the execution of applications both up and out since threads can run task instances within and across processes/nodes. On the other hand, its lack of sharing can cause unnecessary overheads and hinder the scaling up when threads operate on data that could be jointly accessed in shared memory. This trade-off motivated us in studying a way for stream processing applications to leverage shared memory and boost the scale up (before the scale out) while adhering to the widely-adopted and SN-based APIs for stream processing applications. We introduce STRETCH, a framework that maximizes the scale up and offers instantaneous elastic reconfigurations (without state transfer) for stream processing applications. We propose the concept of Virtual Shared-Nothing (VSN) parallelism and elasticity and provide formal definitions and correctness proofs for the semantics of the analysis tasks supported by STRETCH, showing they extend the ones found in common Stream Processing Engines. We also provide a fully implemented prototype and show that STRETCH's performance exceeds that of state-of-the-art frameworks such as Apache Flink and offers, to the best of our knowledge, unprecedented ultra-fast reconfigurations, taking less than 40 ms even when provisioning tens of new task instances.

==> sections/todos.tex <==
\section{stuff}
\subsection{Comments, TO DOs, etc.}

\begin{itemize}
    \item Things noticed after submission
    \begin{enumerate}
        \item since \aggop{} only defines $f_A$ and $f_R$ it implicitely assumes $\psi$ is set to multi.
        \item in the eval we say the latency is the difference of timestamps, but actually that is imprecise... change it or not? Actually the entire definition is wrong...
    \end{enumerate}
    \item Things we might want to do before the final submission
    \begin{enumerate}
        \item given what happened in VLDB for Lachesis, do we need to distinguish a bit between one-at-a-time and micro-batching?
        \item should we use here too the word instance-optimized / specific?
        \item explain in a footnote that the generalized operator uses forward instead of forwardSN forwardVSN for simplicity but of course can use? This are things decided at deploy time, sort of ortoghonal to ours, but good to think a bit, maybe
        \item put a footnote about the lack of $\opmapping$ in A and J because the first time they were not introduced yet?
        \item double-check the RW of the VLDB paper, I think I only took the one from DEBS
        \item Boxplot is missing a piece in Fig 11 and Appendix B
    \end{enumerate}
    \item Consistency related
    \begin{itemize}
        \item check that we use the right term in references, lemma, def, obs, theorem and so on
        \item check when the words process and forward should be replaced by processSN/VSN and forwardSN/VSN. Should not replace inside pseudocode, because those would be for downstream operators X
        \item check order of parameters and actual parameters for general operator and common notation of Aggregate and Join X
        \item double-check appendix table contains everything and in alphabetical order
        \item thread and bucket are old words that should not appear that often X
        % \item I removed the right boundary from the notation of $w$ X
        % \item try to remove $\psi$ (previously $\iota$)? I do not think we can, but maybe we can check later on
        % \item do we need to say tuples are immutable?
        % \item are we using $\delta$? YES
        \item double-check numbering of algorithms because I had to reset the counter X
        \item double-check operator vs operator instance, window vs window instance X
        \item removed ``$s_1$ and one from $s_2$'' when explaining what a Join is. Is it ok? X
        \item its $\tau$ not $ts$ X
        \item use SN/VSN not the extended form once the abbreviations has been created X
        \item $t_o$, not $t_O$ X
        \item check figures in detail
        \item where is the first place in which we mention the appendix table?
        \item \I{} not $I$
    \end{itemize}
    \item Style
    \begin{enumerate}
        \item RULES FOR SUBSCRIPTS AND SUPERSCRIPTS
        \begin{itemize}
            \item subscripts for indexes of instances of operators, or streams. superscripts for indexes in lists (of tuples, of windows and so on)
            \item $j$ for index of operator, except for $j$ operators or if $j$ already taken in that sentence, in that case $i$
            \item $i$ for index of upstream operator or input stream
            \item $\ell$ or $m$ for indexes of lists
            \item $t_{in}$ and $t_{out}$ for generic input and output tuple
         \end{itemize}
        \item parameter versus variable
        \item scale up and scale out no scale-up scale-out
        \item shared memory or shared-memory? Be consistent
        \item dot at end of caption X
        \item no dot at the end of a comment X
        \item check figures tables and so on appear in the right position X
        \item stream processing, not streaming analysis, data streaming X
        \item not always theorems and proofs, some are lemmas I guess? something in appendix? X
        \item specify always proof of what X if not just after
        \item a user not an user
        \item do not call Examples, but rather operators X
        \item maybe function for $f$ and method for pseudocode? X
        \item since not all listings say algorithm, some say example, make sure autoref/ref is consistent X
        % \item it's full of we - remove we
        \item when referencing functions put input params too?
        \item do not use on the one hand on the other hand for stuff that is not related to a trade off X
        \item Watermark or watermark? watermark X
        \item do now use the word section, only autoref X
        \item elastic, not adaptive X
        \item I put source/sink in lower case in the intro X
        \item Algorithm Alg or Alg. X
        \item $=$ or $\leftarrow$? X
        \item process and forward in texttt X
        \item Do not use mathcal with lowercase letters X
        \item check references are there the first time we introduce something (e.g., Apache Flink) X
        \item from problem definition onwards we said we simply use windows for time-based sliding windows X
        \item do not use the word key to refer to ``crucial'' because a key is already used for the parallelization approach X
        \item we do not scale out, we only scale up here. make sure not to oversell X
        \item unify the style used for the function names, some of it is Java like some of it is C like X
        % \item Do we actually use the combined notation for the tuples introduced in preliminaries or not? 
        \item sources vs readers for SG, X - let's be uniform, not writers/entities and so on X
        \item be uniform and mention first $WA$ and then $WS$ X
        \item key values or key-by values? let's decide and be uniform X
    \end{enumerate}
    \item things for the future
    \begin{itemize}
        \item we might want to consider testing STRETCH with Flink too?
    \end{itemize}
\end{itemize}


\subsection{main updates after meeting 21/06/16}
\begin{itemize}
    \item Section 2
    \begin{itemize}
        \item introduced Map, we use it in one corollary
        \item changed the notation for the window, and the window boundaries in preliminaries and section 4 accordingly
        \item added macros for aggregate and join
        \item added a figure about SN parallelism and explained a bit better
        \item clarified that for enforcing determinism for order-sensitive stateful analysis we also want stateful operators to produce timestamp sorted output streams (to support the determinism of their downstream peers).
        \item changed $P$ to \joinpredicate{} for the join predicate, now condition, to avoid confusing with $P$ used for probability.
    \end{itemize}
    \item Section 4
    \begin{itemize}
        \item changed notation for the functions, put them in a table to save some space, you like it?
        \item removed a part (which had comments from Marina) because it was something confusing and then will pop up later on (it was about traver
        \item polished a bit the figure
        \item added the pseudocode of the upstream peer too, we need it to prove correctness
        \item added macros for aggregate and join
        \item updated window notation according to the updated one in Section 2
        \item added a corollary showing Maps can be used for data duplication
        \item introduced \aggplusopinmath{} and \cpop{}.
        \item clarified $P$ is a probability
        \item small example added for the state of $O$.
        \item updated the pseudocode to the more general one (this should be it)
    \end{itemize}
    \item Section 5
    \begin{itemize}
        \item added a very first draft of the section about equivalence SN abd VSN
    \end{itemize}
    \item Section 7
    \begin{itemize}
        \item added a very first draft of the section
    \end{itemize}
\end{itemize}

\subsection{main updates just back from vacations}
\begin{itemize}
    \item Section 2 rewritten entirely
    \begin{itemize}
        \item introduced common representation of stateful operators
        \item rewritten correctness part, please check
        \item updated ready definition (we talk live about the reasons)
    \end{itemize}
\end{itemize}

\subsection{main updates week 31}
\begin{itemize}
    \item Section 2
    \begin{itemize}
        \item polished more
        \item introduced a global assumption that we focus on sliding time windows ($WA<WS$)
    \end{itemize}
    \item Section 3 polished/rewritten theorems up to the introduction of the generalized model
\end{itemize}


\subsection{main updates week 32}
\begin{itemize}
    \item Section 2 3 6
    \begin{itemize}
        \item polished a bit based on section 6 updates.
    \end{itemize}
    \item re-drafted section 3 for the goals of the paper
\end{itemize}

\subsection{main updates week 36/37}
\begin{itemize}
    \item polished examples (working on them) and moved them up
    \item changed a bit intro removing model and moved model down
    \item started working on ESG
    \item changes a bit everywhere to keep things consistent
    \item introduce table of abbreviations
    \item untangling the knots in implementation
\end{itemize}

\subsection{main updates week 38}
\begin{itemize}
    \item fixed the ESG addsources thing
    \item worked more on the examples, realized they need to come actually after explaining scalegate (because of the equijoin)
    \item restructured a bit the SG part
    \item refined proof of correctness for elasticity
    \item starting cleaning implementation
    \item started cleaning evaluation
\end{itemize}

\subsection{main updates week 39}
\begin{itemize}
    \item updated elasticity section to be aligned with implementation section - realized there was a corner case and the problem of who delivers watermarks
    \item worked on implementation section
    \item polished a bit previous comments
    \item significantly polished also section 5 (again because of the work on the implementation section) - added a small theorem
    \item polished more ESG section, need to discuss with Marina: If an \elasticscalegate{} implementation wants to and concurrent calls
\end{itemize}

\subsection{main updates week 40}
\begin{itemize}
    \item introduction, some cosmetics
    \item preliminaries, some cosmetics
    \item problem definition, some cosmetics plus change related to the ``we discuss one stateful operator but it applies to many'' thread
    \item general operator, cosmetics and moved up theorem about watermarks, better fits here and hopefully helps not loosing the thread in the following section
    \item static setups, changed based on the moved theorem (see previous point) + fixed some small inconsistency + polishing
    \item dynamic setups, changed assumptions to conditions (Marina) and cosmetics
    \item implementation, completed first serious draft, now can start polishing iterations
    \item started polishing the modeling subsection (all symbols were old)
\end{itemize}

\subsection{main updates week 41}
\begin{itemize}
    \item moved to TPDS format
    \item major polishing of abstract, intro and preliminaries
    \item first patching of evaluation
    \item we need to discuss the modeling
    \item started gathering scripts and so on to produce graphs
    \item fixed some pending comment
\end{itemize}
